Minkowski Operations of Sets with Application to Robot Localization

This papers shows that using separators, which is a pair of two complementary contractors, we can easily and efficiently solve the localization problem of a robot with sonar measurements in an unstructured environment. We introduce separators associated with the Minkowski sum and the Minkowski difference in order to facilitate the resolution. A test-case is given in order to illustrate the principle of the approach.

==> eptcsdata.tex <==
\providecommand{\firstpage}{34}
\providecommand{\publicationstatus}{E. {\'A}brah{\'a}m and S. Bogomolov (Eds.): 3rd International\\ Workshop on Symbolic and Numerical Methods for Reachability\\ Analysis (SNR 2017)\\
EPTCS 247, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.247.3}{10.4204/EPTCS.247.3}}
\pdfoutput=1

